Critical Motility-Induced Phase Separation in Three Dimensions is Consistent with Ising Universality

Identifying the universality class of critical active phase transitions has been the subject of recent interest and controversy. Resolving these controversies will require robust numerical investigations to determine whether active critical exponents point to novel universality classes or are consistent with established ones. Here, we conduct large-scale computer simulations and a finite-size scaling analysis of the motility-induced phase separation (MIPS) of active Brownian hard spheres in three dimensions (3D), finding that the static and dynamic critical exponents all closely match those of the 3D Ising universality class with a conserved scalar order parameter. This finding is corroborated by a fluctuating hydrodynamic description of the critical dynamics of the order parameter field which flows to the Wilson-Fisher fixed point in three dimensions. Our work suggests that 3D MIPS and likely the entire phase diagram of active Brownian hard spheres is similar to that of molecular passive fluids despite the absence of Boltzmann statistics.

==> custom-commands.tex <==
\usepackage{multirow}

% ******** CUSTOMIZATIONS  ******** %
\DeclareMathAlphabet\mathbfcal{OMS}{cmsy}{b}{n}

%******** FONT FORMATTING ********%
\DeclareMathAlphabet{\mathpzc}{OT1}{pzc}{m}{it}
\DeclareMathAlphabet\mathbfcal{OMS}{cmsy}{b}{n}

\DeclarePairedDelimiter\floor{\lfloor}{\rfloor}
%new command
\newcommand{\xmark}{\ding{55}}%
\newcommand*\diff{\mathop{}\!\mathrm{d}}

%When editing
%\newcommand{\ed}[1]{{\color{blue}#1}}
\newcommand{\ed}[1]{{\color{black}#1}}

\newtheorem{theorem}{Theorem}
\newtheorem{lemma}[theorem]{Lemma}

\makeatletter
\DeclareRobustCommand{\svdots}{%
  \hbox{ }\vbox{%
    \baselineskip 3\p@
    \lineskiplimit \z@
    \kern 1\p@
    \hbox{.}\hbox{.}\hbox{.}%
  }%
  \hbox{ }
}
\makeatother

\makeatletter
\def\overvect@#1#2#3{\vbox{\ialign{##\crcr
       \noalign{\kern-.7pt\nointerlineskip}#1#2\crcr
       \noalign{\kern1pt\nointerlineskip}$\m@th\hfil#2#3\hfil$\crcr}}}
\makeatother
\def\*#1{\mathbf{#1}}
%\newcommand{\todo}[1]{\textcolor{RedViolet}{[ToDo: #1]}}
\newcommand{\fvect}[1]{\overset{\rightarrow}{#1}}
\newcommand{\bvect}[1]{\overset{\leftarrow}{#1}}
\newcommand{\scp}{\mathcal{P}}
\newcommand{\bscp}{\partial \scp}

\DeclareMathOperator\erfc{erfc}
% increase line spacing in matrix environments
\makeatletter
\renewcommand*\env@matrix[1][\arraystretch]{%
  \edef\arraystretch{#1}%
  \hskip -\arraycolsep
  \let\@ifnextchar\new@ifnextchar
  \array{*\c@MaxMatrixCols c}}
\makeatother

% better circled text
\newcommand*\circled[1]{
	\tikz[baseline=(char.base)]{
		\node[shape=circle,draw,inner sep=1pt] (char) {#1};
	}
}
%coloring in math mode
\makeatletter
\def\mathcolor#1#{\@mathcolor{#1}}
\def\@mathcolor#1#2#3{%
  \protect\leavevmode
  \begingroup
    \color#1{#2}#3%
  \endgroup
}
\makeatother

%short arrow that can rotate
\makeatletter
\newcommand{\fixed@sra}{$\vrule height 2\fontdimen22\textfont2 width 0pt\shortrightarrow$}
\newcommand{\shortarrow}[1]{%
  \mathrel{\text{\rotatebox[origin=c]{\numexpr#1*45}{\fixed@sra}}}
}
\makeatother
\makeatletter
\newcommand{\blankarrow}{\textcolor{white}{\shortarrow{1}}}
\makeatother

%boxing characters
\makeatletter
\renewcommand{\boxed}[1]{\text{\fboxsep=.2em\fbox{\m@th$\displaystyle#1$}}}
\makeatother

%small fraction
\newcommand\ddfrac[2]{\frac{\displaystyle #1}{\displaystyle #2}}
%\geometry{margin=1in}

%short to
\newcommand{\shortto}[1][3pt]{\mathrel{%
   \hbox{\rule[\dimexpr\fontdimen22\textfont2-.2pt\relax]{#1}{.4pt}}%
   \mkern-4mu\hbox{\usefont{U}{lasy}{m}{n}\symbol{41}}}}

\def\doubleunderline#1{\underline{\underline{#1}}}

%TikZ code "illustrating" the new "brace"
\newcommand{\newbrace}[1][]{
\begin{tikzpicture}[baseline=-0.5ex]
\draw[#1] (0,0) -- (0.3,0.3);
\draw[#1] (0,0) -- (0.3,-0.3);
\end{tikzpicture}
}

% the optional argument allows you to select the type of arrow 
% you can also customize the "new brace"
\newenvironment{casesnew}[1][->]%
{\;\newbrace[#1]\;\begin{array}{@{}l@{}}}%
{\end{array}}

%Declaring some math operators
\DeclareMathOperator{\Tr}{Tr}
\DeclareMathOperator{\sech}{sech}
\allowdisplaybreaks

\renewcommand{\thefigure}{S.\arabic{figure}}
\renewcommand{\thetable}{S.\arabic{table}}

\usepackage[linesnumbered,ruled,vlined]{algorithm2e}
\DontPrintSemicolon
% Define pseudocode formatting
\renewcommand{\KwSty}[1]{\textnormal{\textcolor{blue!90!black}{\ttfamily\bfseries #1}}\unskip}
\renewcommand{\ArgSty}[1]{\textnormal{\ttfamily #1}\unskip}
\SetKwComment{Comment}{\color{green!50!black}// }{}
\renewcommand{\CommentSty}[1]{\textnormal{\ttfamily\color{green!50!black}#1}\unskip}
\newcommand{\assign}{\leftarrow}
\newcommand{\var}{\texttt}
\newcommand{\FuncCall}[2]{\texttt{\bfseries #1(#2)}}
\SetKwProg{Function}{function}{}{}
\renewcommand{\ProgSty}[1]{\texttt{\bfseries #1}}


%%%%%%%%%%%%%%%%%%%%%%% Wide tilde %%%%%%%%%%%%
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{stackengine}
\usepackage{scalerel}
